ComplexBeat: Breathing Rate Estimation from Complex CSI

In this paper, we explore the use of channel state information (CSI) from a WiFi system to estimate the breathing rate of a person in a room. In order to extract WiFi CSI components that are sensitive to breathing, we propose to consider the delay domain channel impulse response (CIR), while most state-of-the-art methods consider its frequency domain representation. One obstacle while processing the CSI data is that its amplitude and phase are highly distorted by measurement uncertainties. We thus also propose an amplitude calibration method and a phase offset calibration method for CSI measured in orthogonal frequency-division multiplexing (OFDM) multiple-input multiple-output (MIMO) systems. Finally, we implement a complete breathing rate estimation system in order to showcase the effectiveness of our proposed calibration and CSI extraction methods.

==> sec/equations.tex <==
\section{Equations}



\begin{align}
\tilde{H}_{i, j, \tilde{m}} = A_j^{\text{AGC}}[t] \left( | H_{i, j, \tilde{m}}[t] | e^{j \angle H_{i, j, \tilde{m}}[t]} \right) e^{j (\alpha_i^{\text{off}}[t] \tilde{m} + \beta_i^{\text{off}}[t])} \notag
\end{align}

\begin{align}
| \hat{H}_{i, j, \tilde{m}}[t] | 
= \frac{| \tilde{H}_{i, j, \tilde{m}}[t] |}{\frac{1}{M} \sum_{\tilde{m}}|{\tilde{H}}_{i-1, j, \tilde{m}}[t] |}
= \frac{A_j^{\text{AGC}}[t] | H_{i, j, \tilde{m}}[t] | }{A_j^{\text{AGC}}[t] \frac{1}{M} \sum_{\tilde{m}} | H_{i, j, \tilde{m}}[t] |} \notag
\end{align}

\begin{align}
\angle \hat{H}_{i, j, \tilde{m}}[t]  \notag   \\
& = \angle \tilde{H}_{i, j, \tilde{m}}[t] - j((\alpha_{i, j, \tilde{m}'}[t] + \alpha_i^{\text{off}}[t]) \tilde{m} + \beta_{i, j, \tilde{m}'}[t] + \beta_i^{\text{off}}[t]) \notag  \\
& = \angle H_{i, j, \tilde{m}}[t] + (\alpha_i^{\text{off}}[t] \tilde{m} + \beta_i^{\text{off}}[t]) -   \notag \\
& (\alpha_{i, j, \tilde{m}'}[t] \tilde{m} + \beta_{i, j, \tilde{m}'}[t])  - (\alpha_i^{\text{off}}[t] \tilde{m} + \beta_i^{\text{off}}[t])  \notag \\
& = \angle H_{i, j, \tilde{m}}[t] - (\alpha_{i, j, \tilde{m}'}[t] \tilde{m} + \beta_{i, j, \tilde{m}'}[t])
\end{align}

==> sec/preliminaries_short.tex <==
\section{Preliminaries}
In this section, we describe the structure of \gls{csi} as well as the \gls{csi} phase distortion and we explain the phase difference method described in \cite{wang_phasebeat_2017} as basis for the improvements described in Section \ref{sec:pre_select}.
\label{sec:Preliminaries}
\subsection{CSI and CIR in WiFi MIMO OFDM Systems}
Consider an OFDM system operating in a multipath channel.
The transmitter sends training information and the receiver extracts the complex baseband channel state information that can be described as
%The source signal in the time domain is denoted as $s(t)$. 
%After up-conversion to the carrier frequency, the transmitted signal is written as $\tilde{s}(t) = s(t)e^{j2\pi f_c t}$, where $f_c$ is the center carrier frequency.
%At the receiver side, the reflected signal along path $p$ arrives at the receiver with delay $\tau_p$, and accumulates with other paths:
%\begin{align}
%\tilde{r}(t) = \sum_{p=1}^{P} A_p s(t-\tau_p) e^{j2\pi %f_c(t-\tau_p)}
%\end{align}
%where $P$ is the number of paths, $A_p$ is the attenuation on path $p$.
%After down-conversion at the receiver side, here we assume the transmitter and receiver are perfectly synchronized and there is no phase noise, the received signal is:
%\begin{align}
%r(t) 
%&= \tilde{r}(t) e^{j2\pi f_c(-t)} \notag \\
%&= \sum_{p=1}^{P} A_p s(t-\tau_p) e^{j2\pi f_c(-\tau_p)}
%\end{align}
%By comparing source signal $s(t)$ and received $r(t)$, the \gls{csi} can be written as: 
%\begin{align}
%h(t) = \sum_{p=1}^{P} A_p \delta(t-\tau_p) e^{j2\pi f_c(-\tau_p)}
%\end{align}
%where $\delta$ is Dirac delta function.
%If we calculate the DFT of $h(t)$, we transform from delay domain to spectral domain of the channel, which is: 
%\begin{align}
%H(f) = \sum_{p=1}^{P} A_p e^{-j 2 \pi (f-f_c) \tau_p}
%\end{align}
%And by replacing $f$ with $\Delta f \tilde{m}$, we obtain the discrete version of $H(f)$, which is \gls{csi}:
\begin{align}
H_{\tilde{m}} = \sum_{p=1}^{P} A_p e^{-j 2 \pi (\Delta f \tilde{m}-f_c) \tau_p},
\label{equ:pre_csi_multi_path}
\end{align}
%where $\Delta f$ is the subcarrier spacing, $\tilde{m}$ is subcarrier index, 
where $P$ is the number of paths, $A_p$ and $\tau_p$ are the attenuation and delay on path $p$, respectively, $\tilde{m}$ is the subcarrier index, $\Delta f$ is the subcarrier spacing and $f_c$ is the carrier frequency.
Note that $\Delta f \tilde{m}$ is the baseband carrier frequency, which is between $-\frac{B}{2}$ and $\frac{B}{2}$, where $B$ is the bandwidth.
In an OFDM communication system, this channel state information is commonly denoted by a vector $\mathbf{H} = [H_1, H_2, \cdots, H_M]^T$, where $M$ is the number of subcarriers.
%Each entry of $\mathbf{H}$ is a complex number consist of an amplitude $|H_m|$ and a phase $\angle H_m$, representing the channel condition for each subcarrier $m$.
%for the $m$ th subcarrier is described as a complex number $H_m$ consists of the magnitude $|H_m|$ and angle $\angle H_m$ components.
%As shown in (\ref{equ:pre_csi_multi_path}), $H_{\tilde{m}}$ is the superposition of complex numbers $A_p e^{-j 2 \pi (\Delta f \tilde{m}+f_c) \tau_p}$ on each path $p$ . 
Each entry of $\mathbf{H}$ is a function of $\tau_p$, which can be used to estimate the change of $\tau_p$ over time.
%We use $\tilde{m}$ to denote the subcarrier indices, instead of elements in such that $\Delta f \tilde{m}$ is the baseband carrier frequency.

%The vector formed by all $M$ subcarries' $H_m$ is the \gls{csi} $\mathbf{H} = [H_1, H_2, \cdots, H_M]^\top$.
For the WiFi MIMO OFDM case, where there is more than one transmitter (TX) / receiver (RX) antenna pair, the \gls{csi} can be written as a high dimensional array $H_{i, j, \tilde{m}} \in \mathbb{C}^{N_T\times N_R\times M}$, where $N_T$ and $N_R$ are the number of TX and RX antennas, respectively. 
To observe the change in the channel, multiple \gls{csi} snapshots are obtained. 
A \gls{csi} sample set is written as a four-dimensional array $H_{i, j, \tilde{m}}[t] \in \mathbb{C}^{T\times N_T\times N_R\times M}$, where $T$ is the number of snapshots.

\subsection{CSI Phase Distortion and RX Phase Difference}
\label{sec:CSI_phasediff}
In the case where the transmitter and receiver are not synchronized and phase noise is present, \gls{pbd} error, \gls{sfo}, and \gls{cfo} have an influence on the phase component of \gls{csi}.
The \gls{csi} sample set, including these distortion can be described as \cite{speth_optimum_1999}
\begin{align}
\tilde{H}_{i, j, \tilde{m}} = H_{i, j, \tilde{m}} e^{j2\pi ((\xi^{d}_i+\xi^{s}_i) \tilde{m} + \xi^{c}_i + \gamma_i)},
\label{equ:pre_csi_multi_path_offset}
\end{align}
where $\tilde{H}_{i, j, \tilde{m}}$ is the distorted \gls{csi} value for TX antenna $i$, RX antenna $j$ and subcarrier index $\tilde{m}$, $\gamma_i$ is the initial phase offset due to the phase-locked loop (PLL), $\xi^{d}_i$, $\xi^{s}_i$ and $\xi^{c}_i$ are the phase errors from the \gls{pbd} error, \gls{sfo}, and \gls{cfo}, respectively \cite{speth_optimum_1999} for TX~$i$. 
The offset values are identical for all RX antennas on the same receiver at the same snapshot $t$.
The phase components of CSI from TX antenna $i$ to RX antenna $j$ is
\begin{align}
\angle \tilde{H}_{i, j,\tilde{m}} = \angle H_{i, j,\tilde{m}} + ((\xi^{d}_i+\xi^{s}_i) \tilde{m}_i + \xi^{c}_i + \gamma_i )
\label{equ:pre_phase_h1}
\end{align}
In order to eliminate the unknown phase component $((\xi^{d}_i+\xi^{s}_i) \tilde{m} + \xi^{c}_i + \gamma_i )$, the work of \cite{wang_phasebeat_2017} proposed to subtract $\angle \tilde{H}_{i, j',\tilde{m}}$ from $\angle \tilde{H}_{i, j,\tilde{m}}$, and obtain the RX phase difference $\angle \tilde{H}_{i, k,\tilde{m}}$
\begin{align}
\angle \tilde{H}_{i, k,\tilde{m}} =\angle H_{i, j,\tilde{m}} - \angle H_{i, j',\tilde{m}}
\label{equ:pre_phase_diff}
\end{align}
By taking multiple snapshots of $\angle \tilde{H}_{i, k,\tilde{m}}$ over time, we obtain $\angle \tilde{H}_{i, k,\tilde{m}}[t]$. 
According to \cite[Lemma 1]{wang_phasebeat_2017}, when the wireless signal is reflected from the chest of a person with a breathing frequency $f_r$, the true phase of the reflected signal at any antenna of the receiver is also periodic with the same frequency $f_r$.
The phase difference $\angle \tilde{H}_{i, k,\tilde{m}}$, as the linear combination of $\angle H_{i, j, \tilde{m}}$ and $\angle H_{i, j', \tilde{m}}$, contains this periodic component of $f_r$ as well. 

\section{CSI Calibration and Selection}
In this section, we introduce our new calibration method that is used to eliminate phase distortion  from the measurement.
We explain the different sensitivity of the phase to breathing movement between different subcarriers, and introduce a criterion for selecting those sensitive phase components.
\subsection{CSI Calibration: Linear Component Approach}
\label{sec:pre_calib}
Instead of calculating the difference between the phase components on two RX antennas as shown in \cite{wang_phasebeat_2017}, we introduce a calibration method that avoids the need to dedicate one antenna element as a reference and preserves the shape of the \gls{csi}. 
%Different from the self-linear calibration method that has been proposed in \cite{7417517}, we calibrate the phase of one RX antenna using the \gls{csi} phase from another RX antenna.

To this end, we exploit that the phase offsets, as shown in (\ref{equ:pre_phase_h1}), for all RX antennas are identical and are linear functions of the subcarrier index $\tilde{m}$. 
We thus write the term $(\xi_{d}+\xi_{s}) \tilde{m} + \xi_{c} + \gamma$ as $\alpha \tilde{m} + \beta$, which yields 
\begin{align}
\tilde{H}_{j, \tilde{m}} = H_{j, \tilde{m}} e^{j(\alpha \tilde{m} + \beta)}
\end{align}
%Now we assume that the delay spread is small, i.e., that there exists a dominant path between the transmitter and the receiver that has delay $\tau_0$ and amplitude $A_0 \gg A_p$ ($p \neq 0$), and the path reflected on the human chest is the only dynamic path. 
Now we assume that the delay spread is small, i.e., that there is a dominant path between the transmitter and the receiver, and that the path reflected on the human chest is the only dynamic path.
%This assumption is not completely realistic, but it provides valuable insight. 
When the assumption holds, the \gls{csi} phase $\angle H_{j, \tilde{m}'}$ of a small subset of adjacent subcarriers $\tilde{m}'$, shows a linear trend along $\tilde{m}'$, and the linear coefficients are denoted as $\alpha_j'$ and $\beta_j'$. 
With the influence of phase distortion, the linear trend coefficients along $\tilde{m}'$ of $\angle \tilde{H}_{j, \tilde{m}'}$ become $\tilde{\alpha}_j' = \alpha_j' + \alpha$ and $\tilde{\beta}_j' = (\beta_j' + \beta)$, where $\tilde{\alpha}_j'$ and $\tilde{\beta}_j'$ can be obtained from the \gls{csi} phase measurement $\angle \tilde{H}_{j, \tilde{m}}$.
%Then we define the term $\text{lin}(\angle \tilde{H}_{j, \tilde{m}'}) := \tilde{\alpha}_j' \tilde{m} + \tilde{\beta}_j'$.
%With the influence of phase distortion, $\text{lin}(\angle \tilde{H}_{j, \tilde{m}'}) = (\alpha_j' + \alpha) \tilde{m} + (\beta_j' + \beta)$.
We then calibrate the \gls{csi} on RX antenna with index $j+1 \pmod{N_R}$ by multiplying it with $e^{-j (\tilde{\alpha}_j' \tilde{m} + \tilde{\beta}_j')}$.
In the following, we denote $j+1 \pmod{N_R}$ by $j+1$ for simplicity.
After calibration, the calibrated \gls{csi} is written as
%The path reflected on the human chest is the only dynamic  path with index $p_d$, where $p_d \neq 0$. 
%We write the \gls{csi} for RX antenna $j$ as:
%\begin{align}
%\tilde{H}_{j, \tilde{m}}
%= & H_{j, \tilde{m}} e^{j(\alpha \tilde{m} + \beta)} \notag \\
%= &\{A_{0, j}e^{-j 2\pi (\Delta f \tilde{m} - f_c) \tau_{0, j}} \notag \\ 
%+ &\sum_{p \neq 0} A_{p, j} e^{-j 2\pi (\Delta f \tilde{m} - f_c) \tau_{p, j}} \} e^{j(\alpha \tilde{m} + \beta)},
%\end{align}
%where $A_{p, j}$ and $\tau_{p, j}$ are the amplitude and delay for $p$th path and $j$th RX antenna.
%Since we assume that $A_0 \gg A_p$ ($p \neq 0$), the linear phase component of RX antenna $j_a$, $\text{lin}(\angle \tilde{H}_{j_a, \tilde{m}}) = \alpha_{j_a} \tilde{m} + \beta_{j_b}$, can be approximated by $\hat{\alpha}\tilde{m} + \hat{\beta}$, where $\hat{\alpha} \approx -2 \pi \Delta f \tau_{0, j_a} + \alpha$ and $\hat{\beta} \approx 2 \pi f_c \tau_{0, j_a} + \beta$.
%\begin{align}
%\hat{\alpha} \approx -2 \pi \Delta f \tau_{0, j_a} + \alpha
%\end{align}
%\begin{align}
%\hat{\beta} \approx 2 \pi f_c \tau_{0, j_a} + \beta
%\end{align}
%We calibrate \gls{csi} on the neighboured antenna $\tilde{H}_{j_b, \tilde{m}}$ by multiplying it with $e^{-j\text{lin}(\angle \tilde{H}_{j_a, \tilde{m}})} \approx e^{-j(\hat{\alpha}\tilde{m} + \hat{\beta})}$.
%After calibrating the phase, the calibrated \gls{csi} is written as:
%\begin{align}
%\hat{H}_{j_b, \tilde{m}}
%= & H_{j_b, \tilde{m}} e^{j (\alpha \tilde{m} + \beta)} e^{-j( \hat{\alpha}\tilde{m} + \hat{\beta})} \label{equ:calib_all} \\ 
%= & H_{j_b, \tilde{m}} e^{j2\pi (\Delta f \tilde{m} - f_c)\tau_{0,j_a}} \label{equ:calib} \\
%= &  A_{0, j_b} e^{-j 2\pi (\Delta f \tilde{m} -f_c) (\tau_{0, j_b} - \tau_{0, j_a})} \notag \\
%+ & \sum_{p \neq 0} A_{p, j} e^{-j 2\pi (\Delta f \tilde{m} - f_c) \tau_{p, j}}  e^{j 2 \pi (\Delta f \tilde{m}-f_c)\tau_{0, j_a}}
%\label{equ:calib01}
%\end{align}
\begin{align}
\hat{H}_{j+1, \tilde{m}}
=  H_{j+1, \tilde{m}} e^{-j (\alpha_j' \tilde{m} + \beta_j')}
\label{equ:calib01}
\end{align}
%Similarly, we can calibrate $\tilde{H}_{j_a, \tilde{m}}$ with $\text{lin}(\angle \tilde{H}_{j_b, \tilde{m}})$. 
If the signal reflected on the human chest is on the dominant path, i.e., the breathing movement affects $\alpha'_j$ and $\beta'_j$, the phase component of (\ref{equ:calib01}) still contains the term $(\alpha'_{j+1} - \alpha'_{j}) \tilde{m}  + (\beta'_{j+1} - \beta'_{j}) $, which still has periodic part of $f_r$, according to \cite[Lemma 1]{wang_phasebeat_2017}.
In such case, our method shows advantage compared to the similar self-linear calibration method discussed in \cite{Wang_PhaseFi_2015}, where the antenna is calibrated by its own linear phase component which causes the phase term that contains useful breathing rate information to vanish.
On the other hand, if the signal reflected on the human chest is not on the dominant path for both antennas and the dominant path is static over time, the calibrated $\hat{H}_{j+1, \tilde{m}}$ is the true \gls{csi} of antenna $j+1$ multiplied by a term, $e^{-j (\alpha_j' \tilde{m} + \beta_j')}$ that is almost constant over snapshots $t$ for all $\tilde{m}$, as shown in (\ref{equ:calib01}).
From \cite[Lemma 1]{wang_phasebeat_2017}, the phase component of $H_{j, \tilde{m}}[t]$ is periodic with the breathing rate $f_r$, thus the $\hat{H}_{j, \tilde{m}}$ is also periodic with $f_r$, if the dominant path is static.


\subsection{CSI Candidates Selection}
\label{sec:pre_select}
After we have calibrated the \gls{csi}, we further look into the structure of the calibrated \gls{csi} $\hat{H}_{i, j, \tilde{m}}$ for antenna pair $(i, j) $ at subcarrier index $\tilde{m}$. 
We keep assuming that the path reflected by the moving human chest is the only dynamic path $p_d$ in the channel and the rest of the paths are all static across snapshots
\begin{align}
H_{i, j, \tilde{m}}
&= \sum_{p \neq p_d} A_{p, i, j} e^{-j 2\pi (\Delta f \tilde{m} - f_c) \tau_{p, i, j}} \notag \\
&+ A_{p_d, i, j} e^{-j 2\pi (\Delta f \tilde{m} - f_c) \tau_{p_d, i, j}}
\label{equ:channel_model}
\end{align}
\begin{figure}[t]\centering
\subcaptionbox{Stability against noise \label{fig:subsel2}}{
\input{./pics/tikz_subsel_2.tex}
}\quad
\subcaptionbox{Displacement sensitivity \cite{zeng_fullbreathe_2018} \label{fig:subsel1}}{
\input{./pics/tikz_subsel_1.tex}
}
\caption{\gls{csi} on the complex plane for different subcarriers.}
\end{figure}
The superposition of the static paths is a new complex number for each subcarrier, represented by the solid arrows in Fig.~\ref{fig:subsel2}. 
The added dynamic component has a phase that changes as a function of $\tau_{p_d}$, as shown by the dashed arrows. 
$H_{i, j, \tilde{m}}$ is the superposition of the dynamic and static components, resulting in the orange and blue arrows in Fig.~\ref{fig:subsel2} for different $\tilde{m}$.
The amplitude of some \gls{csi} subcarriers is small, shown as the orange line in Fig.~\ref{fig:subsel2}. 
%For such cases, their phase components are very sensitive to \gls{awgn} in the channel, which makes the phase component unstable along time, as shown in the orange curve in Figure~\ref{fig:good_bad2}.
For such cases, their phase is very sensitive to noise, which makes the phase unstable over time.
Moreover, we observe that the deviation of $\angle H_{i, j, \tilde{m}}$ as a function of the dynamic component can be very different even for two subcarriers with very similar magnitude, as shown in Fig \ref{fig:subsel1}.
A similar variation in sensitivity also applies across antennas, depending on the position of the antenna and the human chest \cite{zeng_fullbreathe_2018}.
%Also for the phase difference method, different wavelengths on different subcarriers lead to different sensitivity for breathing signals \cite{wang_phasebeat_2017}. 
%Some of the subcarriers have larger deviation caused by breathing, as shown in Figure~\ref{fig:good_bad1}. 
%Some of the subcarriers have larger deviation caused by breathing. 
%In the work of \cite{wang_phasebeat_2017}, a subcarrier selection method based on the mean absulute deviation (MAD) method is proposed, which selects the subcarrier, whose unwrapped phase along time axis has the second largest MAD value, for respiration rate estimation.

We thus introduce a selection method for the best subcarrier and antenna pair based on the specific variation of the phase over time.
The elements in the candidate set $\{\mathbf{\Phi}:\Phi_{i, j, m}[t] = \angle \hat{H}_{i, j, \tilde{m}}$ for $i\in[1:N_T], k \in [1,N_R]$,  $m \in [1, M]$.
%For the phase difference method, the set is then $\{\mathbf{\Phi}:\Phi_{i, k, m}[t], i\in[1:N_T], k \in [1,N_R-1]$,  $m \in [1, M]\}$, where $\Phi_{i, k, m}[t]$ is the phase difference calculated using (\ref{equ:pre_phase_diff}).

An ideal waveform $\Phi[t]$ for estimating the breathing rate should be smooth and not spiky, and have a large periodic component.
Thus we first normalize $\Phi[t]$ into $\tilde{\Phi}[t]$ such that it has a mean of zero and a variation of one.
We then calculate a score $S$ as a combination of total variation (TV) and the mean absolute deviation (MAD) over the snapshots
\begin{align}
\text{TV}(\tilde{\Phi}[t]) = \frac{1}{T-1} \sum_{t=1}^{T-1} |\tilde{\Phi}[t+1] - \tilde{\Phi}[t]|
\end{align}
\vspace{-0.4cm}
\begin{align}
\text{MAD} (\tilde{\Phi}[t]) = \frac{1}{T} \sum_{t=1}^{T} |\tilde{\Phi}[t] - \mathbb{E} [\tilde{\Phi}[t]]|
\end{align}
The TV is a criterion to check the smoothness of edges of waveforms, and the MAD is a criterion to check the spikyness of a normalized 1D waveform. 
We combine these two criteria into one metric 
\begin{align}
S_{i, j, m} = -\text{TV}(\tilde{\Phi}_{i, j, m}[t]) + \text{MAD}(\tilde{\Phi}_{i, j, m}[t])
\label{equ:TV_mad}
\end{align}
to select the best candidate for further processing.

\subsection{Delay Domain Filter}
\label{sec:delay_filter}
The majority of existing CSI-based breathing estimation methods rely on filtering in the snapshot domain. 
We introduce a method for filtering in delay domain for each snapshot, based on the fact that the \gls{csi} naturally allows for the separation of paths with different delays.
%The channel contains multiple paths reflected on different objects. 
To estimate the breathing rate, we are only interested in the path reflected by the human chest.
However, there exist other, longer paths reflected on both the chest and other objects that we refer to as additional dynamic paths.
%To avoid the influence from such paths in the channel, we introduce delay domain filtering.
%We write the \gls{csi} $H_{\tilde{m}}$ between one antenna pair as :
%\begin{align}
%H_{\tilde{m}} &= \sum_{p \in \{p: \tau_p < \tau_{\text{thr}}\}} A_{p} e^{-j2\pi(\Delta f \tilde{m} -f_c)  \tau_{p}}  \notag\\
%&+ \sum_{p \in \{p: \tau_p \geq \tau_{\text{thr}}\}}  A_{p} e^{-j2\pi(\Delta f \tilde{m} -f_c)  \tau_{p}} 
%\end{align}
%Recall that the IFFT of \gls{csi} is \gls{csi}, which is a function of delay $\tau$.
%We can filter the \gls{csi} in the delay domain and withdraw components with delay $\tau$ larger than a certain threshold $\tau_{\text{thr}}$. 
%Unfortunately, it is impossible to only keep the path reflected on the human chest, because of the low resolution in the delay domain.
%However, with rough prior knowledge of the position range of the person, we can exclude a large number of delay components that are from the additional dynamic paths.
%After filtering out the components with larger delays, the \gls{csi} is transformed back into the spectral domain as $\hat{H'}_{\tilde{m}}$.
%where $\mathcal{F}^{-1}(\cdot)$ is the inverse discrete Fourier transform, $g_{\text{Thr}}(\cdot)$ is the delay domain filter with cut-off delay of $\tau_{\text{Thr}}$, and $\mathcal{F}(\cdot)$ is the discrete Fourier transform.
To this end, we first transform the calibrated \gls{csi} $\hat{H}_{\tilde{m}}$ into a \gls{cir} as a function of $\tau$. We estimate an upper bound $\tau_{\text{max}}$ for the delay of relevant single-reflection paths (based on the size of the room). All \gls{cir} components with a delay $\tau >\tau_{\text{max}}$ are set to zero and the resulting filtered \gls{cir} is transformed back into the frequency domain. 
\begin{align}
\hat{H'}_{\tilde{m}} = \mathcal{F}\left(
\begin{cases}
\mathcal{F}^{-1}(\hat{H}_{\tilde{m}}), & \text{if}\ \tau \leq \tau_{\text{max}} \\
0, & \text{otherwise}
\end{cases}
\right)
\label{equ:delay_filter}
\end{align}
%\begin{figure}[h]
%\input{./pics/tikz_plot_cir_block.tex}
%\end{figure}
